Spatio-temporal extreme event modeling of terror insurgencies

Extreme events with potential deadly outcomes, such as those organized by terror groups, are highly unpredictable in nature and an imminent threat to society. In particular, quantifying the likelihood of a terror attack occurring in an arbitrary space-time region and its relative societal risk, would facilitate informed measures that would strengthen national security. This paper introduces a novel self-exciting marked spatio-temporal model for attacks whose inhomogeneous baseline intensity is written as a function of covariates. Its triggering intensity is succinctly modeled with a Gaussian Process prior distribution to flexibly capture intricate spatio-temporal dependencies between an arbitrary attack and previous terror events. By inferring the parameters of this model, we highlight specific space-time areas in which attacks are likely to occur. Furthermore, by measuring the outcome of an attack in terms of the number of casualties it produces, we introduce a novel mixture distribution for the number of casualties. This distribution flexibly handles low and high number of casualties and the discrete nature of the data through a {\it Generalized ZipF} distribution. We rely on a customized Markov chain Monte Carlo (MCMC) method to estimate the model parameters. We illustrate the methodology with data from the open source Global Terrorism Database (GTD) that correspond to attacks in Afghanistan from 2013-2018. We show that our model is able to predict the intensity of future attacks for 2019-2021 while considering various covariates of interest such as population density, number of regional languages spoken, and the density of population supporting the opposing government.

==> exploratory.tex <==
% !TEX root = main.tex
\section{Exploratory study}
% \section{Preliminaries} % (fold)
% \label{sec:preliminaries}
In this section, we describe the relevant mathematical background that form the basis of typical extreme value analyses. Specifically, the Generalized Extreme Value (GEV) distribution is formulated for block maxima models and the Generalized Pareto distribution (GPD) for threshold based models. 

\subsection{Block maxima models} % (fold)
\label{sub:block_maxima}
Letting $X_1, X_2, \dots, X_n$ be a sequence of independent random variables having a common distribution function $F$, block maxima models focus on the statistical modeling of
$$M_n = \max(X_1, X_2, \dots, X_n),$$
and a \textit{block} is considered a period e.g. monthly or annually that each contain observations of $X_1, \dots, X_n$. 

In practice, the distribution $F$ is unknown. To circumvent this, the Fisher-Tippett-Gnedenko theorem \citep{RN218} states that if there exist a sequence of constants $(a_n,b_n)$ with $a_n>0$, then the limit
$$\lim_{n \to \infty} \mathbb{P} \left( \frac{M_n-b_n}{a_n} \leq z \right) = G(z).$$
Here, if $G$ is non-degenerate then $G$ belongs to one of the Gumbel, Fr\'echet or Weibull distribution families. These three families can be succinctly grouped into the family of the Generalized Extreme Value (GEV) distribution. Specifically, if $Z \sim \hbox{GEV}(\mu,\sigma,\xi)$, then its CDF takes the form
\begin{align} \label{eq:GEV}
	G(z) := \mathbb{P}(Z \leq z) = \exp \left( - \left[ 1 + \xi \left( \frac{z-\mu}{\sigma} \right) \right]^{-1/\xi} \right),
\end{align}
defined on $\{z: 1+ \xi(z-\mu)/\sigma > 0\}$. Here, $\mu \in \mathbb{R}$ is the \textbf{location} parameter, $\sigma >0$ is the \textbf{scale} parameter $\xi \in \mathbb{R}$ is the \textbf{shape} parameter. Furthermore, renormalization implies that 
\begin{align*}
	\mathbb{P}(M_n \leq z) & \approx G\left(\frac{z-b_n}{a_n}\right) \\
	& = G^\ast(z),
\end{align*}
which is another member of the GEV family \citep{RN218}. 

This enables the distribution of \textit{block maxima} (or minima) to be well approximated by distributions from the GEV family, from which maximum likelihood estimation is in general numerically straight-forward to recover the unknown parameters from given data. 
% subsection block_maxima (end)

\subsection{Threshold models} % (fold)
\label{sub:threshold_models}

While distributions from GEV family are subject to favorable asymptotic properties \citep{RN218}, one of the main drawbacks from utilizing the GEV in this  manner is that the data in blocks $X_1, X_2, \dots, X_n$ is often wasted via computation of their maximum (or minimum), frequently resulting in insufficient data for the GEV to be an accurate modeling tool. An alternative approach, which endeavors to utilize data that are observed above a particular threshold, are threshold based models.

Letting $X_1, X_2, \dots, X_n$ again be a sequence of independent random variables having a marginal common distribution function $F$, threshold models define an extreme event $X$ from this sequence as that which exceeds some high threshold $u$. Specifically, its conditional probability is given as 
\begin{align*}
	\mathbb{P}(X>u+x|X>u) = \frac{1-F(u+x)}{1-F(u)} \quad x>0.
\end{align*}
Since in practical applications the distribution $F$ is commonly unknown, an approximation to $\mathbb{P}(X>u+x|X>u)$ is necessary. \cite{RN218} uses the GEV distribution defined in (\ref{eq:GEV}) for large $n$ and $u$, to yield 
\begin{align} \label{eq:gpd_cond}
	\mathbb{P}(X \leq u+x|X>u) = 1 - \left(1 + \frac{\xi x}{\sigma + \xi(u-x)} \right)^{-1/\xi},
\end{align}
defined on $\left\{x: x>0, \left(1 + \frac{\xi x}{\sigma + \xi(u-x)} \right) >0 \right\}$.

Re-parameterizing (\ref{eq:gpd_cond}), the CDF of $X \sim \hbox{GPD}(u,\sigma,\xi)$ is given by 
\begin{align} \label{eq:gpd_cdf}
	\mathbb{P}(X \leq x)  = \begin{cases}
		1 - \left(1 + \frac{\xi(x-u)}{\sigma}\right)^{-1/\xi} & \text{for } \xi \neq 0 \\
		1 - \exp \left( - \frac{x-u}{\sigma}\right) & \text{for } \xi = 0,
	\end{cases}
\end{align}
where the support of $X$ satisfies $x \geq u$ when $\xi \geq 0$ and $u \leq x \leq u-\frac{\sigma}{\xi}$ when $\xi<0$. Similarly to the GEV, $\sigma > 0$ is the \textbf{scale} parameter, $\xi \in \mathbb{R}$ is the \textbf{shape} parameter and $u \in \mathbb{R}$ is the \textit{threshold} or \textbf{location} parameter. 

This enables the distribution of data over a pre-specified threshold or \textit{exceedances} to be well approximated by the GPD, from which maximum likelihood estimation is in general numerically straight-forward to recover the unknown parameters from given data. Analyzing threshold exceedances in this manner are commonly referred to as peaks over threshold (PoT) models. Although these methods typically utilize the data more efficiently than block maxima models, selecting a suitable threshold for which the GPD remains a suitable model, without losing efficiency of the data, is not straightforward and remains an active area of research in this field. 

The interested reader is directed to \cite{RN218} for further information of the GEV distribution, GPD and other extreme valued type constructions. Figures \ref{fig:gev_iraq} and \ref{fig:gpd_iraq} illustrate GEV and GPD fits for the casualties information for Iraq.

 \begin{figure}
	\centering
	\begin{subfigure}{.45\textwidth}
	  \centering
	  \includegraphics[scale=.45]{./Figures/iraq_gev_fit.pdf}
	  \caption{GEV fit Iraq.}
	  \label{fig:gev_iraq}
	\end{subfigure}%
	\begin{subfigure}{.45\textwidth}
	  \centering
	  \includegraphics[scale=.45]{./Figures/iraq_gpd_fit.pdf}
	  \caption{GPD fit Iraq.}
	  \label{fig:gpd_iraq}
	\end{subfigure}
	% \caption{Plots of global casualties during 1970-2018.}
	% \label{fig:plots_all}
\end{figure}

% \section{Extreme value analysis} % (fold)
% \label{sec:country_level}

% In order to analyze the viability of extreme value analysis across all space-time terrorism attacks, it is important to assess its performance first at the \textit{country level}, i.e. in large regions of space where attacks can be viewed independently of other regions and where temporal structures can be emphasized. In this section, we look at the five most (historically) attacked countries, as described in Section \ref{sec:introduction}, within specific time periods that do not suffer too greatly from the data limitations highlighted in Section \ref{ssub:data_challenges}. The countries analyzed in this section are summarized in Table \ref{table:countries_time_periods}. 

% In Section \ref{sub:block_maxima_cl}, we use the block maxima approach and fit a GEV distribution to monthly maxima of casualties, both spatially and temporally. In Section \ref{sub:points_over_threshold_cl}, we use the peaks over threshold approach and fit a GPD distribution to threshold exceedances, including a discussion on threshold selection methods.

% \begin{table}
% \centering
% 	\begin{tabular}{||c | c||} 
% 		\hline
% 		\textbf{Country} & \textbf{Time period} \\ 
% 		\hline
% 		\hline
% 		Iraq & 2004-2018 \\ 
% 		\hline
% 		Pakistan & 2002-2018 \\
% 		\hline
% 		Afghanistan & 2003-2018 \\
% 		\hline
% 		India & 2002-2018 \\
% 		\hline
% 		Colombia & 1977-1995 \\
% 		\hline
% 	\end{tabular}
% \caption{}
% \label{table:countries_time_periods}
% \end{table}

% % \subsection{Extreme value analysis} % (fold)
% % \label{sub:extreme_value_analysis}

% \subsection{Analysis of block maxima} % (fold)
% In order to use the GEV distribution to GTD country level data, we computed the \textit{monthly maxima} of casualties over the time periods considered. A monthly block for this dataset was favored over a daily block, which would have resulted in too many null observations, and a yearly block which would have resulted in too few data points. Using these datasets, the standard GEV distribution can be fitted using maximum likelihood estimation, and goodness of fit plots (specifically probability, quantile, density and return levels) that use the maximum likelihood estimated parameters, can be assessed. 

% Figures \ref{fig:iraq_gev}-\ref{fig:ind_gev} show the monthly maxima with the corresponding GEV goodness of fit plots for Iraq, Pakistan, Afghanistan, India and Colombia. All countries seem to suggest a good distributive fit with the (standard) GEV, although Pakistan and Colombia yield the poorest of quantile fits. 
% \label{sub:block_maxima_cl}
% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/iraq_max_casualties.png}
% 	  \caption{Iraq maximum casualties.}
% 	  \label{fig:iraq_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.6]{./Figures/iraq_gev_fit.pdf}
% 	  \caption{Iraq GEV plots.}
% 	  \label{fig:iraq_gev_fit}
% 	\end{subfigure}
% 	\caption{Maximum monthly casualties in Iraq and its corresponding GEV goodness of fit plots.}
% 	\label{fig:iraq_gev}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/pak_max_casualties.png}
% 	  \caption{Pakistan maximum casualties.}
% 	  \label{fig:pak_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.6]{./Figures/pak_gev_fit.pdf}
% 	  \caption{Pakistan GEV plots.}
% 	  \label{fig:pak_gev_fit}
% 	\end{subfigure}
% 	\caption{Maximum monthly casualties in Pakistan and its corresponding GEV goodness of fit plots.}
% 	\label{fig:pak_gev}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/afg_max_casualties.png}
% 	  \caption{Afghanistan maximum casualties.}
% 	  \label{fig:afg_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.6]{./Figures/afg_gev_fit.pdf}
% 	  \caption{Afghanistan GEV plots.}
% 	  \label{fig:afg_gev_fit}
% 	\end{subfigure}
% 	\caption{Maximum monthly casualties in Afghanistan and its corresponding GEV goodness of fit plots.}
% 	\label{fig:afg_gev}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/ind_max_casualties.png}
% 	  \caption{India maximum casualties.}
% 	  \label{fig:ind_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.6]{./Figures/ind_gev_fit.pdf}
% 	  \caption{India GEV plots.}
% 	  \label{fig:ind_gev_fit}
% 	\end{subfigure}
% 	\caption{Maximum monthly casualties in India and its corresponding GEV goodness of fit plots.}
% 	\label{fig:ind_gev}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/col_max_casualties.png}
% 	  \caption{Colombia maximum casualties.}
% 	  \label{fig:col_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.6]{./Figures/col_gev_fit.pdf}
% 	  \caption{Colombia GEV plots.}
% 	  \label{fig:col_gev_fit}
% 	\end{subfigure}
% 	\caption{Maximum monthly casualties in Colombia and its corresponding GEV goodness of fit plots.}
% 	\label{fig:col_gev}
% \end{figure}

% Spatially, attack data can be analyzed for its clustering or inhibitive properties. Estimates of Ripley's K and pair correlation functions are provided in Figures \ref{fig:gev_ripleys_k} and \ref{fig:gev_pcf} for each country previously studied and highlight the high spatial clustering of attacks in comparison to a homogeneous (uniform) spatial Poisson process. Furthermore, the GEV data within the time period 2002-2018 in the Middle East region is plotted in Figure \ref{fig:ripleys_gev}, which further highlights attack clusters around cities and regions of known political conflict. 

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{.5\textwidth}
% 	  \includegraphics[scale=.26]{./Figures/gev_ripleys_k.png}
% 	  \caption{GEV: Ripley's K function.}
% 	  \label{fig:gev_ripleys_k}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\textwidth}
% 	  \includegraphics[scale=.26]{./Figures/gev_pcf.png}
% 	  \caption{GEV: Pair correlation functions.}
% 	  \label{fig:gev_pcf}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 		\centering
% 		\includegraphics[scale=.4]{./Figures/gev_all_map.png}
% 		\caption{GEV data plotted spatially.}
% 		\label{fig:ripleys_gev}
% 	\end{subfigure}
% 	\caption{Spatial analyses of block maxima (GEV) attack data.}
% \end{figure}
% % subsubsection block_maxima (end)

% \subsection{Analysis of peaks over threshold} % (fold)
% \label{sub:points_over_threshold_cl}

% In order to use the GPD distribution to GTD country level data, we first observe the casualties that exceed the $99\%$, $95\%$ and $90\%$ empirical quantiles over the time periods considered. We then use mean residual life and parameter stability plots to determine a suitable threshold for each country. Using these datasets, the standard GPD distribution can be fitted using maximum likelihood estimation, and goodness of fit plots (specifically probability, quantile, density and return levels) that use the maximum likelihood estimated parameters, can be assessed. 

% Figure \ref{fig:all_ex} shows the exceedances of the data at three empirical quantiles. It is evident that, even in the case of the $99\%$ quantile, the data seems to extremely heavy tailed (with many points lying above this quantile), providing first evidence of the suitability of PoT models. 

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/iraq_exceedants.png}
% 	  \caption{Iraq exceedances.}
% 	  \label{fig:iraq_ex}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/pak_exceedants.png}
% 	  \caption{Pakistan exceedances.}
% 	  \label{fig:pak_ex}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{.5\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/afg_exceedants.png}
% 	  \caption{Afghanistan exceedances.}
% 	  \label{fig:afg_ex}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/ind_exceedants.png}
% 	  \caption{India exceedances.}
% 	  \label{fig:ind_ex}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/col_exceedants.png}
% 	  \caption{Colombia exceedances.}
% 	  \label{fig:col_ex}
% 	\end{subfigure}
% 	\caption{Observed exceedances (on log scale) at the $90\%$ (black), $95\%$ (blue) and $99\%$ (red) quantiles.}
% 	\label{fig:all_ex}
% \end{figure}

% In order to continue with the GPD fitting, it is necessary to define the threshold $u$ for each country, for which an attack is considered extreme. Threshold selection is indispensable when using the GPD, since choosing a threshold which is too low may invalidate the Generalized Pareto distributive assumption on the tails of the observed data, while picking a threshold which is too large is likely to encounter maximum likelihood convergence issues due to too few points exceeding it. Although there are many methods \citep{RN231} to aid us in doing so, we follow \cite{RN218} and use graphical tools. The three main plots we can consider are the mean residual life plot, and the GPD scale and shape stability plots. 

% The mean residual life (MRL) plot utilizes the fact that for $X \sim \hbox{GPD}(u_0,\sigma_{u_0}, \xi)$, $\mathbb{E}(X-u|X>u) = \frac{\sigma_{u_0} + \xi u}{1-\xi}$, for all $u > u_0, \; \xi<1$. This expectation is a linear function of $u$. This is important since the unbiased estimate of $\mathbb{E}(X-u|X>u)$, the mean of all excesses above $u$, are therefore expected to change linearly in $u$ at levels of $u$ for which the GPD is appropriate. This is exactly what the MRL computes over different values of $u$. 

% On the other hand, the scale and shape stability plots use the fact that if the GPD is valid at threshold $u_0$, then excesses of a higher threshold $u>u_0$ also follow a GPD with identical shape parameter $\xi$ and scale parameter $\sigma_u = \sigma_{u_0} + \xi(u-u_0)$. This implies that the \textit{modified} scale parameter $\sigma^\ast = \sigma_u - \xi u$ is constant with respect to $u$. The shape and scale stability plots therefore provide maximum likelihood estimates for the shape and modified scale parameters across different values of $u$, with a suitable threshold $u_0$ being that which the parameter estimates are approximately constant above.

% A threshold can then be chosen once the MRL becomes approximately linear and/or the shape/scale stability plots become constant. As stated above, it is important to understand the bias/variance trade-off between picking a large enough threshold to render the GPD appropriate, while also having sufficient data above it for model fitting and selection. 

% Figures \ref{fig:iraq_ts} - \ref{fig:col_ts} show the MRL and shape/scale stability plots for the countries considered. From these plots, it is evident that the GPD in general provides a good fit at low thresholds with most countries, with the exception of Pakistan, from which a poorer fit is observed. In this case, a larger threshold is required to ensure parameter stability. 

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/iraq_mrl.png}
% 	  \caption{Mean residual life plot.}
% 	  \label{fig:iraq_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/iraq_param_stability.png}
% 	  \caption{Parameter stability plots.}
% 	  \label{fig:iraq_param_stab}
% 	\end{subfigure}
% 	\caption{Iraq: Threshold selection tools.}
% 	\label{fig:iraq_ts}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/pak_mrl.png}
% 	  \caption{Mean residual life plot.}
% 	  \label{fig:pak_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/pak_param_stability.png}
% 	  \caption{Parameter stability plots.}
% 	  \label{fig:pak_param_stab}
% 	\end{subfigure}
% 	\caption{Pakistan: Threshold selection tools.}
% 	\label{fig:pak_ts}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/afg_mrl.png}
% 	  \caption{Mean residual life plot.}
% 	  \label{fig:afg_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/afg_param_stability.png}
% 	  \caption{Parameter stability plots.}
% 	  \label{fig:afg_param_stab}
% 	\end{subfigure}
% 	\caption{Afghanistan: Threshold selection tools.}
% 	\label{fig:afg_ts}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/ind_mrl.png}
% 	  \caption{Mean residual life plot.}
% 	  \label{fig:ind_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/ind_param_stability.png}
% 	  \caption{Parameter stability plots.}
% 	  \label{fig:ind_param_stab}
% 	\end{subfigure}
% 	\caption{India: Threshold selection tools.}
% 	\label{fig:ind_ts}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/col_mrl.png}
% 	  \caption{Mean residual life plot.}
% 	  \label{fig:col_max_cas}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.45]{./Figures/col_param_stability.png}
% 	  \caption{Parameter stability plots.}
% 	  \label{fig:col_param_stab}
% 	\end{subfigure}
% 	\caption{Colombia: Threshold selection tools.}
% 	\label{fig:col_ts}
% \end{figure}

% The thresholds selected for each country using these plots is given in Table \ref{table:gpd_thresholds_cl}.  The corresponding GPD goodness of fit plots for Iraq, Pakistan, Afghanistan, India and Colombia are shown in Figure \ref{fig:all_gpd}. All countries seem to suggest a good distributive fit with the (standard) GPD.

% \begin{table}[h]
% \centering 
% 	\begin{tabular}{||c | c|}
% 		\hline
% 		\textbf{Country} & \textbf{Threshold}\\ 
% 		\hline
% 		\hline
% 		Iraq & $100$ \\ 
% 		\hline
% 		Pakistan & $60$ \\
% 		\hline
% 		Afghanistan & $50$ \\
% 		\hline
% 		India & $20$ \\
% 		\hline
% 		Colombia & $10$ \\
% 		\hline
% 	\end{tabular}
% \caption{}
% \label{table:gpd_thresholds_cl}
% \end{table}  

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/iraq_gpd_fit.pdf}
% 	  \caption{Iraq GPD fit.}
% 	  \label{fig:iraq_gpd}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/pak_gpd_fit.pdf}
% 	  \caption{Pakistan GPD fit.}
% 	  \label{fig:pak_gpd}
% 	\end{subfigure}\\[1ex]
% 	\begin{subfigure}{.5\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/afg_gpd_fit.pdf}
% 	  \caption{Afghanistan GPD fit.}
% 	  \label{fig:afg_gpd}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/ind_gpd_fit.pdf}
% 	  \caption{India GPD fit.}
% 	  \label{fig:ind_gpd}
% 	\end{subfigure}\\[1ex]
% 	\end{figure}
% 	\begin{figure}[ht]\ContinuedFloat
% 	\begin{subfigure}{\linewidth}
% 	  \centering
% 	  \includegraphics[scale=.5]{./Figures/col_gpd_fit.pdf}
% 	  \caption{Colombia GPD fit.}
% 	  \label{fig:col_gpd}
% 	\end{subfigure}
% 	\caption{GPD goodness of fit plots.}
% 	\label{fig:all_gpd}
% \end{figure}

% Similarly to the GEV data, estimates of Ripley's K and pair correlation functions are provided in Figures \ref{fig:gpd_ripleys_k} and \ref{fig:gpd_pcf} for each country using GPD data and analogously highlight the high spatial clustering of attacks. The data within the same time period in the Middle East region shown in Figure \ref{fig:ripleys_gpd}, however, highlights a much greater amount of data available through a PoT approach. 

% \begin{figure}[h]
% 	\centering
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/gpd_ripleys_k.png}
% 	  \caption{GPD: Ripley's K function.}
% 	  \label{fig:gpd_ripleys_k}
% 	\end{subfigure}%
% 	\begin{subfigure}{.5\textwidth}
% 	  \centering
% 	  \includegraphics[scale=.26]{./Figures/gpd_pcf.png}
% 	  \caption{GPD: Pair correlation functions.}
% 	  \label{fig:gpd_pcf}
% 	\end{subfigure}
% 	\begin{subfigure}{\textwidth}
% 	\centering
% 	\includegraphics[scale=.4]{./Figures/gpd_all_map.png}
% 	\caption{GPD data plotted spatially.}
% 	\label{fig:ripleys_gpd}
% 	\end{subfigure}
% 	\caption{Spatial analyses of points over threshold (GPD) attack data.}
% \end{figure}

==> exploratory_copy.tex <==
% !TEX root = main.tex
\section{Exploratory descriptors}

==> results_2.tex <==
% !TEX root = main.tex
\section{Results}
We first validate our inference method on simulated data to demonstrate its accuracy in estimating all unknown parameters of the model. We then apply the method to infer the underlying process of terrorism events on two real datsets acquired from the Global Terrorism Database. The first, studies and predicts future terror events in Afghanistan based upon event data between 2013 and 2019. The second, studies terror patterns between 1999-2007 in India and Pakistan and investgates the predictability of the Mumbai attacks in November 2008. 

\subsection{Simulations}
% \begin{figure}
% 	\centering
% 	\includegraphics[width=.45\textwidth]{./Figures/post_mu.png}
% 	\includegraphics[width=.45\textwidth]{./Figures/traceplot_mu.png}
% 	\caption{MCMC estimation with a simulated realization of a spatio-temporal Hawkes process}
% 	\label{fig:MCMC}
% \end{figure}

\subsection{Examples in GTD database}
Here we utilize our method on two datasets in the GTD: Afghanistan between 1999-2007 and India/Pakistan 1999-2007. 

The raw event data from the GTD for each of these two studies contains some missing values in the form of unknown event times (as days), locations (as latitude/longitude values) and covariates. To deal with this, the data used was preprocessed and missing values interpolated to generate a full dataset. Further, times were jittered uniformly across the day to become a continuous variable needed in the model. Latitude and longitude values were also jittered using a Gaussian distribution centered around their given coordinate with a small standard deviation  , thereby adding some randomness to event data determined to the nearest city of true event locations. To be able to use the aforementioned methodology, we standardize the times $t_i \in [0,T]$, locations $\bs_i \in W$ and marks $m_i \in M$ to be within $(0,1)$ and post-scale the resulting spatio-temporal intensity by the area $T \times W$. 
\subsubsection{Afghanistan 2013-2019} % (fold)
\label{ssub:afghanistan_2013_2019}
In this study, over $10^4$ terror events were collected, data preprocessed and the analysis run. To be able to predict future events in 2020 and 2021, the time variable $T$ was extended to December 31st 2021. 

To be able to incorporate terror patterns that show dependence between spatial locations and casualties, an initial MCMC run represented the covariance for $f(\cdot)$ as the space-time separable function
$$K(\bx,\by) = \exp \left(-\frac{|t_\bx-t_\by|^2}{2l_t^2} \right) \left(1 + \frac{||(\bs_x,m_x) - (\bs_y,m_y)||^2}{2\alpha_s l_s}\right)^{-\alpha_s},$$
additionally positing a shorter relative time scale for terror excitation. When run, however, prohibitively large values for $\alpha_s$ deemed the covariance function 
$$K(\bx,\by) = \exp \left(-\frac{|t_\bx-t_\by|^2}{2l_t^2} \right) \exp \left(\frac{||(\bs_x,m_x) - (\bs_y,m_y)||^2}{2l_s^2}\right)$$
more suitable to be used for this dataset. 
\begin{figure}[b]
\centering
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2013.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2014.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2015.png}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2016.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2017.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2018.png}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2019.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2020.png}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{./Figures/afg_2021.png}
\end{subfigure}
\caption[short]{A beautiful, well written caption}
\end{figure}

% \subsubsection{India/Pakistan 1999-2007} % (fold)
% \label{ssub:india_pakistan_1999_2007}

% % subsubsection india_pakistan_1999_2007 (end)
% subsubsection afghanistan_2013_2019 (end)

% \begin{figure}
% \centering
% \includegraphics[scale=.52]{./Figures/pakafg_0708.pdf} 
% \includegraphics[scale=.52]{./Figures/pakind_08.pdf}
% \caption{Marked spatio-temporal intensity estimate of attacks 2007-2008.} 
% \label{fig:results1}
% \end{figure}



